Good-looking but Lacking Faithfulness: Understanding Local Explanation Methods through Trend-based Testing

While enjoying the great achievements brought by deep learning (DL), people are also worried about the decision made by DL models, since the high degree of non-linearity of DL models makes the decision extremely difficult to understand. Consequently, attacks such as adversarial attacks are easy to carry out, but difficult to detect and explain, which has led to a boom in the research on local explanation methods for explaining model decisions. In this paper, we evaluate the faithfulness of explanation methods and find that traditional tests on faithfulness encounter the random dominance problem, \ie, the random selection performs the best, especially for complex data. To further solve this problem, we propose three trend-based faithfulness tests and empirically demonstrate that the new trend tests can better assess faithfulness than traditional tests on image, natural language and security tasks. We implement the assessment system and evaluate ten popular explanation methods. Benefiting from the trend tests, we successfully assess the explanation methods on complex data for the first time, bringing unprecedented discoveries and inspiring future research. Downstream tasks also greatly benefit from the tests. For example, model debugging equipped with faithful explanation methods performs much better for detecting and correcting accuracy and security problems.

==> sections/abstract.tex <==
\begin{abstract}
While enjoying the great achievements brought by deep learning (DL), people are also worried about the decision made by DL models, since the high degree of non-linearity of DL models makes the decision extremely difficult to understand. Consequently, attacks such as adversarial attacks are easy to carry out, but difficult to detect and explain, which has led to a boom in the research on local explanation methods for explaining model decisions. In this paper, we evaluate the faithfulness of explanation methods and find that traditional tests on faithfulness encounter the random dominance problem, \ie, the random selection performs the best, especially for complex data. To further solve this problem, we propose three trend-based faithfulness tests and empirically demonstrate that the new trend tests can better assess faithfulness than traditional tests on image, natural language and security tasks. We implement the assessment system and evaluate ten popular explanation methods.
Benefiting from the trend tests, we successfully assess the explanation methods on complex data for the first time, bringing unprecedented discoveries and inspiring future research. Downstream tasks also greatly benefit from the tests. For example, model debugging equipped with faithful explanation methods performs much better for detecting and correcting accuracy and security problems. 
\end{abstract}

==> sections/evaluation.tex <==
\section{Design of Faithfulness Tests}\label{sec:evaluation}

%\todo{It lacks a figure to illustrate the overall process}
%In order to assess the faithfulness of explanation methods, we design new tests and also compare the results with traditional tests. 

In this section, we first provide a high-level definition of faithfulness. Then we briefly introduce traditional evaluation methods and design three trend-based tests, \ie, the evolving-model-with-backdoor test (EMBT), partial-trigger test (PTT), and evolving-model test (EMT), to assess the faithfulness of explanation methods.
% In this section, we first briefly introduce traditional evaluation methods, and then design three trend-based tests, \ie, the evolving-model-with-backdoor test (EMBT), partial-trigger test (PTT), and evolving-model test (EMT), to assess the faithfulness of explanation methods.
The basic idea of the trend tests is to verify how well the known trends correlate with the explanation’s trends. We use natural and backdoor data to create trends during the training and testing phases. In particular, EMBT and PTT create known trends by implanting backdoors into target models. Then, EMBT and PTT assess the explanation results in the training and testing phases, respectively. EMT uses the natural trend in the training phase without backdoor implanting.
%\hjw{The three tests cover intrusive and non-intrusive modes, training and testing phases. EMBT and PTT create known model trends through intrusive backdoors during training and testing, respectively. To ensure their conclusions are transferable to clean models, we also present EMT tested on clean models. We measure the faithfulness of the explanation methods by evaluating the correlation of trends between the explanation results and the known trends.} 
% and also compare the results with traditional tests.
%We designed a faithfulness assessment system for explanation methods. In the system, we designed three new tests, including the evolving-model-with-backdoor test (EMBT), partial-trigger test (PTT), and evolving-model test (EMT), all of which will be introduced in detail later. 

%We also implement traditional evaluation methods for comparison, and empirically verify the existence of the OOD problem. 
These three new tests provide a comprehensive assessment with both clean and backdoor models, which can overcome the OOD problem encountered with the traditional evaluation methods.
 %They are the most comprehensive assessments, containing both clean and backdoor models.
Our experiments comprehensively explore the influencing factors of explanation methods (\eg, data complexity, model complexity and parameters).
% We use multiple metrics for property analysis under these factors, as shown in Table~\ref{eva:metrics}.
Superior to the traditional assessments~\cite{LEMNA,EuroSPSurvey}, our proposed tests can well cope with complex datasets, resulting in new observations and a better understanding. 
% \hjw{Further, trend tests can also promote the development of secure and trustworthy models.}
% of explanation methods.
% have poor support for complex datasets, but our proposed tests are still valid. Thus, we have new observations and deeper understanding on the explanation methods.

% \begin{table}
% 	\caption{Influencing factors, properties and indicators considered in the experiment. $\Delta{P_{target}}$ represents the change of prediction score. }\label{eva:metrics} 
% 	\centering
% 	\scriptsize
% 	\begin{tabular}{c|c|c|c|}
%     \cline{2-4}
%      & \textbf{Factors} & \textbf{Property} & \textbf{Indicator} \\ \hline
%     \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{External}}} & Data Complexity & Faithfulness & $\Delta{P_{target}}$, PCC \\ \cline{2-4} 
%     \multicolumn{1}{|c|}{} & Model Complexity & Faithfulness & $\Delta{P_{target}}$, PCC \\ \hline
%     \multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Internal}}} & Parameters & Sensitivity & Intersection rate \\ \cline{2-4} 
%     \multicolumn{1}{|c|}{} & Run-time randomness & Stability & Intersection rate \\ \hline
% 	\end{tabular}
% \end{table}

% In this paper, we perform assessments on explanation methods, using multiple indicators for property analysis under external and internal influencing factors, as shown in Table~\ref{eva:metrics}. The external factors include data complexity and model complexity. For data complexity, we consider both the size of the data and the number of channels, while for model complexity, we mainly consider the number of trainable parameters of the model. Internal factors include the parameters of the explanation method itself and the run-time randomness. We propose three properties: static faithfulness, sensitivity and stability, to analyze the above mentioned influencing factors. The change in the class probability and intersection rate are used to measure these properties. We introduce each properties and the assessment criteria in the following.

% We designed a measurement system which includes static and dynamic metrics. In the static measurement, we divide the influencing factors of the explanatory method into internal and external factors, which contain four dimensions: data complexity, model complexity, adjustable parameters and run-time randomness. 
% % Note that data and model complexity are related. Complex data usually requires more complex models to achieve better accuracy. In the comparison experiments of data and model complexity, we will use data and models of different complexity to test and observe the performance of different explanatory methods. 
% We define properties such as static fidelity, sensitivity, stability, and efficiency to observe the influencing factors, and use metrics such as delta of confidence, backdoor coverage rate, intersection rate, and average running time to measure the impact quantitatively. 

% In our experiments, we found that the delta of confidence used for static fidelity measurement has poor support for complex data and models due to the fact that the test samples are OOD. To overcome this limitation, we designed the dynamic fidelity as a complement. We use dynamic model tests, dynamic loss test, dynamic data test to measure dynamic fidelity. We find that our proposed dynamic fidelity measurements can better represent the consistency between explanatory results and model behavior. We find that the gradient-based methods are more sensitive to the change of the model. A variety of datasets and models are used to ensure the diversity of the explanatory targets and the generalizability of the experimental results. Other datasets, classification models and explanatory methods can be used in our measurement system.

\subsection{Problem Definition}
An explanation method explains the model decision. However, the results of different explanation methods are not consistent, as shown in Figure~\ref{fig:demo_figure_1}. Therefore, we focus on evaluating the faithfulness of the explanation methods, \ie, how well the explanation behaviors correlate with the model decision behaviors. Below we present a high-level definition of faithfulness and briefly introduce the differences between traditional tests and our proposed trend tests.

\begin{mydef}
(Faithfulness) Given a model $\mathcal{M}$ and an explanation method $\mathcal{E}$. We define faithfulness as the correlation $\rho$ between M's behavior $\mathbf{\hat{M}}$ and the E's behavior $\mathbf{\hat{E}}$.
%\kai{why using different symbols? -- M's behavior}
\end{mydef}

% \begin{mydef}
% \hjw{(Faithfulness) Given a model behavior $\mathbf{B}$ and an explanation result $\mathbf{E}$. $\mathbf{B}$ and $\mathbf{E}$ could be single-element or multi-element sets. We define the faithfulness as $FFN=\rho_{B,E}$. $\rho$ is the correlation function.}
% \end{mydef}

Different faithfulness assessment methods quantify the correlation $\rho$, the model behavior $\mathbf{\hat{M}}$, and the explanation behavior $\mathbf{\hat{E}}$ in different ways. The traditional tests use the model output probability to depict the model behavior, \ie, $\mathbf{\hat{M}}=\mathcal{M}(\mathbf{X})$, where $\mathbf{X}$ is the model input. The explanation behavior is the explanation result of $\mathcal{M}(\mathbf{X})$, \ie, $\mathbf{\hat{E}}=\mathcal{E}(\mathbf{X},\mathcal{M}(\mathbf{X}))$. Traditional tests generate perturbation samples by modifying the important features tagged by the explanation result $\mathbf{\hat{E}}$. The correlation between $\mathbf{\hat{M}}$ and $\mathbf{\hat{E}}$ is measured by the change in the model output probability before and after the modification: $\rho=\mathcal{M}(\tau(\mathbf{X},\mathbf{\hat{E}}))-\mathcal{M}(\mathbf{X})$. $\tau(\mathbf{X},\mathbf{\hat{E}})$ represents the modification function. For example, in the reduction test, $\tau$ is deleting important features tagged by $\mathbf{\hat{E}}$. In trend tests, the model decision behavior and explanation behavior are both sequence, \ie, $\mathbf{\hat{M}}=\{m_i|i\in[0,n],n\in \mathbf{N^+}\}$,  $\mathbf{\hat{E}}=\{e_i|i\in[0,n],n\in \mathbf{N^+}\}$. For example, in EMBT, $\mathbf{\hat{M}}$ is the target label accuracy of the intermediate models recorded during backdoor training; $\mathbf{\hat{E}}$ is the overlapping area between the explanation results of the intermediate models and the backdoor features. The trend tests assess faithfulness by calculating the Pearson correlation coefficient between $\mathbf{\hat{M}}$ and $\mathbf{\hat{E}}$. We will explain the meaning of $\mathbf{\hat{M}}$ and $\mathbf{\hat{E}}$ in detail (see Section~\ref{sec:traditionaltests} and \ref{sec:trendtests}).

\subsection{Traditional Tests}\label{sec:traditionaltests}
To evaluate the faithfulness of explanation methods, traditional tests usually measure the change in prediction scores by mutating the identified important features. We adopt four commonly used tests, including synthesis test~\cite{LEMNA}, augmentation test~\cite{LEMNA} and reduction test~\cite{LEMNA, EuroSPSurvey}.
% and backdoor trigger coverage test~\cite{backdoorxai}. 
In the synthesis test, we only retain the important features ($\mathbf{IF}$) of the test sample marked by the explanation methods and add them on an all black image to form the synthetic sample. Then the difference of target label scores between the synthetic sample and the all black image could indicate the ``importance'' of the identified features (We denote the difference of target label scores by $\rho$). Figure~\ref{fig:test_vis}(a) and (b) show an example of the original test sample and the corresponding synthetic sample of synthesis test, respectively. Intuitively, $\rho$ will increase after $\mathbf{IF}$ are added on the all black image.
In the augmentation test, we randomly select an augmentation sample with a different label from the test samples (see Figure~\ref{fig:test_vis}(c)) from the test set. Then we add IF to the augmentation sample and observe the change of the prediction score ($\rho$). If $\mathbf{IF}$ is valid, $\rho$ is expected to increase.
In the reduction test, we remove $\mathbf{IF}$ from the test sample (see Figure~\ref{fig:test_vis}(d)) and observe $\rho$. In the reduction test, $\rho$ is expected to decrease if $\mathbf{IF}$ are valid. 
% while in the synthesis test and augmentation test, $\Delta P_{target}$ is expected to increase if $F$ are valid.
% In the backdoor-trigger-coverage test, we first train a model that contains a backdoor. Then we generate a test sample by adding the backdoor trigger, and let the explanation method identify the features $\mathbf{IF}$. Since the trigger could be used as the ground-truth of $\mathbf{IF}$, we assess the faithfulness by measuring the overlapped area between $\mathbf{IF}$ and the trigger. 

\begin{figure}
    \setlength{\abovecaptionskip}{4pt}
    \setlength{\belowcaptionskip}{0pt}
    \centering
	\includegraphics[width=0.3\textwidth]{figs/exp_test_vis.pdf}
	\caption{Examples of synthesis test, augmentation test and reduction test. Features with the top 10\% importance scores tagged by the explanation method are considered as important features.}\label{fig:test_vis}
	\vspace{-2mm}
\end{figure}

%Traditional metrics include traditional faithfulness, sensitivity and stability. Traditional faithfulness measures the behavior of a model in terms of changes in classification probability with the basic idea that the greater the change in classification probability of a model, the more important the changed input features are. We have implemented four traditional faithfulness metrics: synthesis test, augmentation test, reduction test and backdoor trigger coverage test. The first three tests refer to Guo \etal~\cite{LEMNA}.
%% , with the difference that we use the change in confidence of the generated test sample in the original classification, rather than the probability that the generated test sample maintains the original classification. The change in confidence is more appropriate in our experiments. 
%Examples of the first three tests are shown in Figure~\ref{fig:test_vis}. The lase test is refer to Lin \etal ~\cite{backdoorxai}. 


%The synthetic sample retains only the important features of the test sample tagged by the explanations, and the remaining features are deleted. The synthetic test calculates the difference of the target label score between the synthetic sample and the test sample. The augmentation test takes a randomly selected augmentation sample from the test set with a different label from the test sample, and overlays the important features of the test sample tagged by explanations onto the augmentation sample. The augmentation test calculates the change in the target label of the augmentation sample before and after adding the important features of the test sample. The reduction test removes important features tagged by the explanations from the test sample, and then calculates the change in target label scores before and after the removal. The backdoor coverage rate test calculates the intersection rate of important features tagged by the explanations with the ground-truth backdoor features.

% In addition to faithfulness, we also evaluate the sensitivity and stability of explanation methods. For a given method, we change its parameters and make explanations for the same input instance. Then the method with different parameters will output different features (e.g., $F_0$, $F_1$, ..., $F_n$). We calculate the overlapped area (i.e., $O$) between these features. The larger the $O$, the lower the sensitivity of the method to parameters. 
% Regarding stability, we measure the impact of randomness on the explanation methods. Some MAE methods need to perturb samples randomly. As a result, different executions of the same methods could generate different features. Again, we calculate the overlapped area (i.e., $O$) between these features. The larger the $O$, the better the stability of the method.

%Sensitivity and stability are used to measure the effects of the adjustable parameters and run-time randomness respectively. They are both quantified by the intersection rate. Sensitivity and stability compares the results of the same explanatory methods run with different parameters or multiple runs with the same parameters respectively. 

\subsection{Trend-based Tests}\label{sec:trendtests}

%We introduce evolving-model-with-backdoor test (EMBT), partial-trigger test (PTT), and evolving-model test (EMT) in this section. 
% As mentioned by BAM~\cite{BAM}, 
The main problem of traditional tests is the OOD samples produced by the tests, which makes the model produce uncertain scores and invalidates the tests. To solve this problem, we design three trend-based tests. The intuition is: instead of using features to mutate samples, we generate a set of samples with a certain ``trend''. Then we let the explanation methods mark important features and check whether the features follow the trend. By measuring the correlation, we can assess the faithfulness of explanation methods. 
%\hjw{Figure~\ref{fig:embt_vis}, \ref{fig:ptt_vis} and \ref{fig:emt_vis} only show cases to help understand the meaning of trend tests. The complete experimental results are in Section~\ref{sec:measurement}.}

%The intuition of the three tests is to describe the behavior of a model by its known dynamic trend. 
%One explanation method that can accurately conform to the dynamic trend is considered to be faithful to the model.
%If the explanation conforms to this dynamic trend, we consider that the faithfulness of the explanation method to be high.

\vspace{2mm}
\noindent\textbf{Evolving-Model-with-Backdoor Test (EMBT).} 
To explain a given model, EMBT adds a backdoor to the model and records the intermediate models in the training process. OOD is that the data distribution for model testing deviates from that for model training~\cite{defood}. The backdoor samples are within the distribution learned by the model, thus solving the OOD problem. The attack success rates of these models form a trend. 
% \hjw{It should be noted that the model may not learn the whole backdoor features. Therefore, directly calculating the overlapped area between the important features marked by the explanation methods can also introduce errors. Backdoor samples are fed during model training, enabling the data that the model learns and locally explained have the same distribution in trend tests.}
In particular, EMBT 
% leverages a $4\times{4}$ white square as the trigger to 
insert a backdoor into the pre-trained model through incremental training~\cite{badnets}. We also evaluate the impact of backdoor in the experiments and give recommendations on backdoor selection (See Section~\ref{subsec:traditionvstrend}). During the training process, EMBT records the intermediate model in every $c$ epochs. Then we could get a set of models $\mathbf{M}=\{M_0,...,M_n\}$. The model $M_0$ is the pre-trained clean model, and $M_i$ is the intermediate model generated in the epoch $i\times{c}$. For a given input instance, EMBT stamps the trigger on the input and measures the probability of the target label on the models $\mathbf{M}$. Suppose the result is $\mathbf{P}_{target}=\{P_0, P_1, ... , P_n\}$. EMBT uses $\mathbf{P}_{target}$ to quantify the model behavior. Figure ~\ref{fig:embt_vis} shows how the probability of the target label changes during the poisoning training process. We can clearly see that there is a trend of $\mathbf{P}_{target}$ drawn with a black line.

\begin{figure}
    \setlength{\abovecaptionskip}{2pt}
    \setlength{\belowcaptionskip}{0pt}
    \centering
	\includegraphics[width=0.45\textwidth]{figs/backdoor_acc_training_process.pdf}
	\caption{EMBT Examples. Saliency's backdoor coverage is more related to ResNet18's backdoor accuracy, with PCC of 0.979, while LIME gets a lower PCC as 0.607.}\label{fig:embt_vis}
	\vspace{-4mm}
\end{figure}

Later, EMBT uses an explanation method to mark the important features on the models $\mathbf{M}$. For each model $M_i$, we can calculate the overlapped area (denoted as $o_i$) between the marked features and the backdoor trigger features (denoted as $t$). We calculate the trigger coverage $s_i=o_i/|t|$. For the $n+1$ models, we could generate a sequence $\mathbf{S}=\{s_0,...,s_n\}$. EMBT uses $\mathbf{S}$ to quantify the explanation behavior. For example, in Figure~\ref{fig:embt_vis}, the solid red line shows the sequence. In this way, we use the two trends $\mathbf{P}_{target}$ and $\mathbf{S}$ to evaluate the faithfulness of the explanation method. 
To measure the correlation between two trends, we employ the Pearson correlation coefficient (PCC)~\cite{pearson}, which is known for calculating the correlation between two variables. PCC is also widely used in the field of deep learning to measure the consistency between the two trends~\cite{pccdl1,pccdl2}.
%\hjw{As we know, the Pearson correlation coefficient (PCC)~\cite{pearson} is famous for calculating the correlation between two variables, and can be widely used to measure the consistency between two trends in deep learning~\cite{pccdl1,pccdl2}.} 
So we calculate PCC:
$$\rho(\mathbf{P}_{target},\mathbf{S})=\frac{cov(\mathbf{P}_{target},\mathbf{S})}{\sigma_{\mathbf{P}_{target}}\sigma_{\mathbf{S}}},$$
where $cov(\mathbf{P}_{target}, \mathbf{S})$ denotes covariance between $\mathbf{P}_{target}$ and $\mathbf{S}$, $\sigma_{\mathbf{P}_{target}}$ and $\sigma_{\mathbf{S}}$ denotes standard deviation of $\mathbf{P}_{target}$ and $\sigma_{\mathbf{S}}$, respectively.
A high value of $\rho(\mathbf{P}_{target},\mathbf{S})$ shows the two trends are consistent, which demonstrates the explanation results are faithful. 
% For example, in Figure~\ref{fig:embt_vis}, the solid black line shows the trend of target label's probability. The solid red line shows the trend of Saliency's backdoor coverage rate and the PCC is 0.979. The other dotted red line shows the trend of LIME's backdoor coverage rate whose PCC is 0.607. The results show that Saliency which has higher faithfulness is more correlated with the solid black line.
For example, we feed backdoor data to the recorded intermediate models and get explanations with Saliency and LIME, respectively. Then the backdoor coverage rate of the top 10\% important features is calculated. The solid red line in Figure~\ref{fig:embt_vis} shows the change in the backdoor coverage rate of Saliency during poisoning training, and the PCC between the solid red line and the black line is 0.979. The other dotted red line shows the change in the backdoor coverage rate of LIME, while the PCC between the dotted red line and the black line is 0.607. We can also see from Figure~\ref{fig:embt_vis} that the solid red line is more similar to the black line than the dotted red line, indicating that PCC correctly reflects the correlation between the two trends. Note that Figure~\ref{fig:embt_vis} only shows an example. We also perform a detailed evaluation of other explanation methods in Section~\ref{sec:measurement}.

%EMBT continues training with a backdoor on a pre-trained model, and records the intermediate model during training. The success rate of backdoor attack of the model gradually increase as shown in Figure~\ref{fig:embt_vis}. 
%We explain a test input on all intermediate models and calculate the backdoor coverage rate for the significant features tagged by the explanations. The known trend in EMBT is the change in the success rate of backdoor attacks. The trend to be verified is the change in backdoor coverage rate tagged by the explanation results as the poisoning training proceeds. Then EMBT calculates the consistency of the above two trends.

%The definition of EMBT is as follows: given a test input $X$ and a series of models $\mathbf{M}=\{M_0,...,M_n\}$ recorded at intervals during backdoor model training. $M_0$ is a pre-trained clean model. If the model is recorded every $j$ epochs, $M_i$ is the model of epoch $i\times{j}$. With the model sequence $\mathbf{M}$, we can get the backdoor attack success rate sequence $Backdoor\_Acc\_Seq=\{Backdoor\_Acc_0,...,Backdoor\_Acc_n\}$ and the backdoor coverage rate sequence $Coverage\_Rate\_Seq =\{Coverage\_Rate_0,...,Coverage\_Rate_n\}$. Then, we assess the faithfulness of the explanation method by the Pearson correlation coefficient between the backdoor attack success rates and the backdoor coverage rate of the explanation results: 
%$$r(X,Y)=\frac{cov(X,Y)}{\sigma_{X}\sigma_{Y}},$$
%where $cov(X,Y)$ denotes covariance between X and Y, $\sigma_X$ denotes standard deviation of X, $X=Backdoor\_Acc\_Seq$ and $Y=Coverage\_Rate\_Seq$.

\vspace{2mm}
\noindent\textbf{Partial-Trigger Test (PTT).} 
Similar to EMBT, PTT uses the backdoor trigger to create the trend. Assume that the model has been backdoored in EMBT. For the input instance to explain, PTT covers the input with part of the trigger (e.g., 10\%-100\%) as shown in Figure~\ref{fig:ptt_data_vis}. We record the trigger coverage as a sequence $\mathbf{S}=\{tc_0,...,tc_n\}$. Then for the generated inputs, we feed them to the model and record the probability of the target label $\mathbf{P}_{target}=\{P_0, P_1, ... , P_n\}$. Similar to EMBT, PTT uses $\mathbf{P}_{target}$ and $\mathbf{S}$ to quantify the model behavior and the explanation behavior, respectively. The black line in Figure~\ref{fig:ptt_vis} shows the probability corresponding to the triggers in Figure~\ref{fig:ptt_data_vis}. From the figure, we can find that, as the proportion of the trigger increases, the prediction score also increases. We also calculate the PCC ($\rho(\mathbf{S}, \mathbf{P}_{target})$) to measure the consistency. 
For example, we generate the test samples with the different partitions of backdoor features and then feed them to the model to get the outputs. The black line in Figure~\ref{fig:ptt_vis} shows the probability of the target label as the trigger proportion increase. With the outputs of the model, we can get the explanation and the backdoor coverage rate of Saliency and IG. Lastly, PCC between the probability of the target label and the backdoor coverage rate can be calculated. The solid red line in Figure~\ref{fig:ptt_vis} shows the backdoor coverage rate of Saliency as the trigger proportion increases. The PCC between the solid red line and the black line is -0.880. The dotted red line is the backdoor coverage rate of IG, whose PCC is 0.948. As can be seen, the dotted red line is more correlated with the black line than the solid red line. 

\begin{figure}
    \setlength{\abovecaptionskip}{4pt}
    \setlength{\belowcaptionskip}{0pt}
    \centering
	\includegraphics[width=0.42\textwidth]{figs/dynamic_data_vis.pdf}
	\caption{Examples of PTT data sequence, made from 10\% to 100\% of the trigger features covered on a clean sample.}\label{fig:ptt_data_vis}
	\vspace{-2mm}
\end{figure}

\begin{figure}
    \setlength{\abovecaptionskip}{2pt}
    \setlength{\belowcaptionskip}{0pt}
    \centering
	\includegraphics[width=0.45\textwidth]{figs/backdoor_score_diff_trigger.pdf}
	\caption{PTT Examples. IG's backdoor coverage curve is more related to ResNet18's accuracy curve, with PCC of 0.948, while Saliency gets a lower PCC as -0.880. }\label{fig:ptt_vis}
	\vspace{-2mm}
\end{figure}

\begin{figure}
    \setlength{\abovecaptionskip}{2pt}
    \setlength{\belowcaptionskip}{0pt}
    \centering
	\includegraphics[width=0.45\textwidth]{figs/delta_loss_training_process.pdf}
	\caption{EMT Examples. Saliency’s $\Delta{F}$ sequence is more related to ResNet50's $\Delta{L}$, with PCC of 0.814, while KS has a lower PCC as 0.286.}\label{fig:emt_vis}
	\vspace{-2mm}
\end{figure}

%PTT implants partial trigger (10\%-100\%) on a clean test input, as shown in Figure~\ref{fig:ptt_data_vis}. Its backdoor attack target label score in the backdoor model with trigger should rise with the proportion of trigger features, as shown in Figure~\ref{fig:ptt_vis}. The known trend in PTT is the change in the backdoor target label score and the trend to be verified is the change in the backdoor coverage rate of the test data.

%The definition of PTT is as follows: given a model $M$, a series of data $\mathbf{X}=\{X_1,...,X_n\}$ with different proportion of trigger features. With the data sequence $X$, we can get the sequence of backdoor target label score $P_{target} =\{P_1,...,P_n\}$ and the backdoor coverage sequence $Coverage\_Rate\_Seq =\{Coverage\_Rate_1,...,Coverage\_Rate_n\}$. Then, we measure the PTT by the Pearson correlation coefficient between the sequence of backdoor attack target label score and backdoor coverage rate of the explanation results: 
%$$r(P_{target},Coverage\_Rate\_Seq).$$

% \begin{table*}[]
% 	\caption{Impact of data complexity on explanation methods assessed by traditional faithfulness tests. The abbreviations are $Syn$:synthetic test, $Aug$: augmentation test, $Red$: reduction test, $Cov$: backdoor-coverage-test, IG: Integrated Gradient, SG: SmoothGrad, DL: DeepLIFT, KS: Kernel Shap.}\label{eva:impactofdatacomplexity} 
% 	\centering
% 	\scriptsize
% 	\begin{tabular}{|c|c||c|c||c|c||c|c||c|c|} \hline
% 	\textbf{Dataset} & \textbf{Method} & $Syn$ & Random & $Aug$ & Random & $Red$ & Random & $Cov$ & Random \\ \hline
% 	\multirow{6}{*}{MNIST} & Saliency & 61.60\% & 6.24\% & 17.41\% & 0.31\% & 50.58\% & 0.94\% & 73.34\% & 3.28\% \\ \cline{2-10} 
%      & IG & 88.51\% & 6.28\% & 24.96\% & 0.24\% & 91.27\% & 0.75\% & 49.51\% & 3.37\% \\ \cline{2-10} 
%      & SG & 85.65\% & 6.86\% & 25.99\% & 0.34\% & 77.57\% & 0.71\% & 78.56\% & 3.49\% \\ \cline{2-10} 
%      & DL & 87.42\% & 6.44\% & 23.67\% & 0.50\% & 90.96\% & 0.72\% & 44.68\% & 3.54\% \\ \cline{2-10} 
%      & KS & 10.62\% & 6.66\% & 0.54\% & 0.37\% & 2.51\% & 0.80\% & 5.56\% & 3.38\% \\ \cline{2-10} 
%      & LIME & 79.61\% & 6.13\% & 16.70\% & 0.53\% & 72.32\% & 0.84\% & 68.84\% & 3.44\% \\ \hline
%     \multirow{6}{*}{CIFAR10} & Saliency & 0.81\% & -0.88\% & 1.08\% & 1.52\% & 53.11\% & 65.73\% & 10.94\% & 4.59\% \\ \cline{2-10} 
%      & IG & 5.84\% & 0.21\% & 2.54\% & 2.23\% & 56.58\% & 65.76\% & 45.92\% & 4.34\% \\ \cline{2-10} 
%      & SG & 5.16\% & -0.41\% & 1.63\% & 2.06\% & 41.91\% & 65.94\% & 84.09\% & 4.46\% \\ \cline{2-10} 
%      & DL & 0.76\% & -0.09\% & 2.91\% & 2.01\% & 60.80\% & 66.22\% & 36.54\% & 4.79\% \\ \cline{2-10} 
%      & KS & -0.11\% & -0.61\% & 1.78\% & 2.10\% & 67.15\% & 65.74\% & 7.36\% & 4.49\% \\ \cline{2-10} 
%      & LIME & 9.67\% & -0.92\% & 1.62\% & 2.06\% & 25.69\% & 66.83\% & 15.20\% & 4.56\% \\ \hline
%     \multirow{5}{*}{Tiny ImageNet} & Saliency & 1.20\% & 0.63\% & 0.35\% & 0.21\% & 66.94\% & 65.98\% & 30.33\% & 2.04\% \\ \cline{2-10} 
%      & IG & 0.98\% & 0.68\% & 0.49\% & 0.26\% & 55.46\% & 65.95\% & 32.88\% & 2.02\% \\ \cline{2-10} 
%      & SG & 3.00\% & 0.60\% & 0.62\% & 0.26\% & 59.17\% & 65.77\% & 74.99\% & 2.04\% \\ \cline{2-10} 
%      & DL & 3.02\% & 0.49\% & 0.48\% & 0.27\% & 65.88\% & 65.77\% & 31.94\% & 2.01\% \\ \cline{2-10} 
%      & LIME & 5.09\% & 0.60\% & 0.41\% & 0.22\% & 43.13\% & 65.95\% & 74.90\% & 2.03\% \\ \hline
% 	\end{tabular}
% \end{table*}

\vspace{2mm}
\noindent\textbf{Evolving-Model Test (EMT).} 
EMT uses the value of the loss function to create the trend without using any backdoor. In particular, EMT records the intermediate models $\mathbf{M}=\{M_0,...,M_n\}$ during the model training process for every $c$ epochs, and also records the corresponding loss values $\mathbf{L} =\{l_0,...,l_n\}$. $M_0$ is the model with untrained random initialization parameters, and the loss value should be large.
% With the training process going on, the loss values gradually decrease,
The magnitude of the change in the loss value during the training responds to the magnitude of the change in the model. The solid black line in Figure~\ref{fig:emt_vis} shows this trend. 
%\hjw{Generally, the EMT can intercept the middle stage of the training process as the trend to be measured.}
% This trend is affected by the adjustment strategy of learning rate, in this paper we adopt momentum, weight decay and cosine annealing strategy. It leads to a change in the loss value that generally falls and then rises and then falls again, corresponding to the start-fast learning-fitting phase of the models, as shown in Figure~\ref{fig:emt_vis}.
Then for a given input, we use the explanation method to mark important features in terms of the $n+1$ models. As a result, we obtain a feature sequence: $\mathbf{F}=\{F_0, ..., F_n\}$. When the loss value becomes stable, the obtained features should also become stable. So we measure and compare the two trends: changes of loss values, and changes of ``important features''. Again, we calculate the PCC: $\rho(\Delta \mathbf{L},\Delta \mathbf{F})$, 
where $\Delta \mathbf{L}=\{|l_{1}-l_{0}|,...,|l_n-l_{n-1}|\}$ and $\Delta \mathbf{F}=\{1-|F_{1} \cap F_{0}|/|F_0|,..., 1-|F_n \cap F_{n-1}|/|F_{n-1}|\}$. $|F_{1} \cap F_{0}|$ represents the number of common features in both $F_{1}$ and $F_{0}$. Sometimes, we do not need to start from the first epoch. We could choose the epoch where the training of the model starts to be stable. EMT uses $\Delta \mathbf{L}$ and $\Delta \mathbf{F}$ to quantify the model behavior and the explanation behavior, respectively.
%where $\Delta L=\{|l_{t}-l_{t-1}|,...|l_n-l_{n-1}|\}$ and $\Delta F=\{|F_{t} \cap F_{t-1}|/|F_0|,..., |F_n \cap F_{n-1}|/|F_0|\}$. $|F_{t} \cap F_{t-1}|$ represents the number of common features in both $F_{t}$ and $F_{t-1}$. $F_t$ is the epoch where the training of the model becomes stable.
For example, we calculate $\Delta \mathbf{L}$ of the recorded intermediate models. The black line in Figure~\ref{fig:emt_vis} shows the change of $\Delta \mathbf{L}$ during training. Then we explain each recorded intermediate model with Saliency and KS. In order to get the $\Delta \mathbf{F}$, we calculate the dissimilarity of the explanations between the current model and the next recorded model. The solid red line and the dotted red line show the $\Delta \mathbf{F}$ of Saliency and KS, respectively, during training. The PCC between the solid red line and the black line is 0.814, while the PCC between the dotted red line and the black line is 0.286. As shown in Figure~\ref{fig:emt_vis}, the solid red line is more correlated with the black line, but the dotted red line remains unchanged.



\vspace{2mm}
\noindent\textit{Remark: relationship between EMBT, PTT and EMT.
The common idea behind all three tests is that they all use trends to assess explanation methods. EMBT and PTT build trends by implanting backdoors into a given DL model. EMBT focuses on the training phase and measures the attack success rate (ASR) trend during training; PTT focuses on the testing phase and calculates the ASR trend when different proportions of backdoor features are used in the trigger. Differently, EMT utilizes clean models without backdoors. It focuses on the loss-change trend of clean model training, which quantifies the change of models. We measure the faithfulness of different trends by calculating the PCC between the known trends and the trends of the explanation results. In short, EMBT and PTT focus on backdoor model training and testing, respectively, while EMT focuses on clean model training.}
%The basic idea of the trend tests is to verify how well the known trends correlate with the explanation's trends. We use natural and backdoor data to create trends during the training and testing phases. During training, EMBT focuses on the attack success rate (ASR) trend of incremental backdoor model training, and EMT focuses on the loss-change trend of clean model training. Loss-change is used to quantify model-change. During testing, PTT focuses on the ASR trend of data containing different proportions of backdoor features. %Unfortunately, we cannot access the trends of the clean model during testing, so we have no test of the clean model in this phase. 



%EMT records intermediate models during the clean training of the model, and the loss function of these intermediate models on the training set largely decreases gradually with the number of iterations, as shown in Figure~\ref{fig:emt_vis}. The known trend in EMT is the change in the loss during model training and the trend to be verified is the change in the explanation results. In EMT, we use the absolute value of the difference between the loss values in adjacent models and the intersection rate of the explained results in adjacent models to represent the known trend and the trend to be verified, respectively.

%The definition of EMT is as follows: given a test input $X$, a series of models $\mathbf{M}=\{M_0,...,M_n\}$ recorded at intervals during model training. $M_0$ is the model with untrained random initialization parameters. With the model sequence $\mathbf{M}$, we can get the loss sequence $Loss\_Seq=\{Loss_1,...,Loss_n\}$ and the sequence of the explanation results $E\_Seq=\{E_1,...,E_n\}$. Then we compute $\Delta Loss=\{Loss_2-Loss_1,...Loss_n-Loss_{n-1}\}$ and $\Delta E=\{E_2-E_1,...E_n-E_{n-1}\}$. The EMT is measured by Pearson correlation coefficient: 
%$$r(\Delta Loss,\Delta E).$$

% \subsection{Traditional Metrics}

% Traditional metrics includes traditional faithfulness, sensitivity and stability. Traditional faithfulness measures the behavior of a model in terms of changes in classification probability with the basic idea that the greater the change in classification probability of a model, the more important the changed input features are. We have implemented four traditional faithfulness metrics: synthesis test, augmentation test, reduction test and backdoor trigger coverage test. The first three tests refer to Guo \etal~\cite{LEMNA}.
% % , with the difference that we use the change in confidence of the generated test sample in the original classification, rather than the probability that the generated test sample maintains the original classification. The change in confidence is more appropriate in our experiments. 
% Examples of the first three tests are shown in Figure~\ref{fig:test_vis}. The lase test is refer to Lin \etal ~\cite{backdoorxai}. 

% \begin{figure}
%     \centering
% 	\includegraphics[width=0.35\textwidth]{figs/exp_test_vis.pdf}
% 	\caption{Examples of synthesis test, augmentation test and reduction test. Features with the top 10\% importance scores tagged by the explanatory method are considered as important features.}\label{fig:test_vis}
% \end{figure}

% The synthetic sample retains only the important features of the test sample tagged by the explanations, and the remaining features are deleted. The synthetic test calculates the difference of the target label score between the synthetic sample and the test sample. The augmentation test takes a randomly selected augmentation sample from the test set with a different label from the test sample, and overlays the important features of the test sample tagged by explanations onto the augmentation sample. The augmentation test calculates the change in the target label of the augmentation sample before and after adding the important features of the test sample. The reduction test removes important features tagged by the explanations from the test sample, and then calculates the change in target label scores before and after the removal. The backdoor coverage rate test calculates the intersection rate of important features tagged by the explanations with the ground-truth backdoor features.

% Given a target sample $X=\{x_1,...,x_n\}$, target label Y and a randomly generated index sequence $T=\{t_1,...,t_k\}$ for comparison. $F_Y$ is the confidence that F classifies X as Y.The explanatory method gives the top $k$ most important features of $X$ as $Z=\{z_1,...,z_k\}$. $z_i$ denotes the position index of the $i^{th}$ feature in $X$.

% \noindent\textbf{Synthesis test:} Given a baseline sample $B=\{b_1,...,b_n\}$. For image data, $Y$ is an all-black image; for text data, $Y$ is an all\ $<$unk$>$ sequence. Let the synthetic sample $S=\{s_1,..,s_n\}$ and the random synthetic sample $S'=\{s'_1,..,s'_n\}$ satisfy the following equation: 

% \begin{multicols}{2}
% \begin{equation}\nonumber
% s_i=\begin{cases}
%         x_i & if\ i\in Z \\
%         b_i & else
%     \end{cases}
% \end{equation}\break
% \begin{equation}\nonumber
% s'_i=\begin{cases}
%         x_i & if\ i\in T \\
%         b_i & else
%     \end{cases}
% \end{equation}
% \end{multicols}

% We then compute fidelity in synthesis test by measuring the change in confidence of the synthetic sample $S$ and the random synthetic sample $S'$ on the target label Y, \ie $Syn(X)=F_Y(S)-F_Y(B)$. The random synthesis test is $Syn'(X)=F_Y(S')-F_Y(B)$.

% \noindent\textbf{Augmentation test:} We randomly draw an irrelevant sample $Q=\{q_1,...,q_n\}$ from the test set. Irrelevant means that the ground-truth label of $Q$ is different from that of the target sample $X$. Let the augmentation sample $A=\{A_1,..,A_n\}$ and the random augmentation sample $A'=\{a'_1,..,a'_n\}$ satisfy the following equation: 
% \begin{multicols}{2}
% \begin{equation}\nonumber
% a_i=\begin{cases}
%         x_i & if\ i\in Z \\
%         q_i & else
%     \end{cases}
% \end{equation}\break
% \begin{equation}\nonumber
% a'_i=\begin{cases}
%         x_i & if\ i\in T \\
%         q_i & else
%     \end{cases}
% \end{equation}
% \end{multicols}
% Similar to synthetic test, we measure the validity in augmentation test by calculating $Aug(X)=F_Y(A)-F_Y(Q)$. The random augmentation test is $Aug'(X)=F_Y(A')-F_Y(Q)$.

% \noindent\textbf{Reduction test:} Given a reference value $u$, which is taken as 0 for image data and $<$unk$>$ for text data, let the reduction sample $R=\{r_1,..,r_n\}$ and the random reduction sample $R'=\{a'_1,..,a'_n\}$ satisfy the following equation: 
% \begin{multicols}{2}
% \begin{equation}\nonumber
% r_i=\begin{cases}
%         u & if\ i\in Z \\
%         x_i & else
%     \end{cases}
% \end{equation}\break
% \begin{equation}\nonumber
% r'_i=\begin{cases}
%         u & if\ i\in T \\
%         x_i & else
%     \end{cases}
% \end{equation}
% \end{multicols}
% Similar to synthetic test, we measure the validity in reduction test by calculating $Red(X)=F_Y(X)-F_Y(R)$. The random reduction test is $Red(X)=F_Y(X)-F_Y(R')$.

% \noindent\textbf{Backdoor pattern coverage test:} We believe that the previous three tests are not sufficient as the distribution of the generated data may differ significantly from that of the training set leading to a significant drop in confidence, but this does not prove the high fidelity of the explanatory method. In general, we are unable to calculate the accuracy of the explanatory method directly, because we cannot know the truly important features for the model. Therefore, we propose to exploit poisoning attacks for creating a biased dataset with truly important features. The bias originates from the backdoor pattern whose location is the truly important features. The backdoor patterns we used in the experiment is shown in Figure~\ref{fig:backdoor_vis}. Suppose we inject the backdoor pattern location at $P=\{p_1,...,p_k\}$, which accounts for a total of $k$ features. Then the backdoor pattern coverage can be computed as followed:
% $$Cov=\frac{|P\cap{Z}|}{k}$$

% \begin{figure}
%     \centering
% 	\includegraphics[width=0.48\textwidth]{figs/exp_backdoor_vis.pdf}
% 	\caption{Examples of samples with backdoor patterns. The white square is the backdoor trigger.}\label{fig:backdoor_vis}
% \end{figure}

% \subsubsection{Similarity}

% Similarity compares horizontally the cases in which the results of different explanatory methods appear to have the same and opposite explanatory results. In the experiment, similarity is used to explore the following questions: 1) Are integrated explanatory methods mutually corroborative? 2) Under what circumstances are the results of different explanatory methods highly similar? 3) Under what circumstances are the results of different explanatory methods less similar? 

% Sensitivity and stability are used to measure the effects of the adjustable parameters and run-time randomness respectively. They are both quantified by the intersection rate. Sensitivity and stability compares the results of the same explanatory methods run with different parameters or multiple runs with the same parameters respectively.

% The intersection rates include isotropic intersection rate and anisotropic intersection rate. Assume that $Z_1=\{z_{11},...,z_{1m}\}$ and $Z_2=\{z_{21},...,z_{2m}\}$ are the results of different explanatory methods. The isotropic intersection rate can be calculated as followed: 

% $$Sim_{iso}=\frac{Z_1[1:k]\cap{Z_2[1:k]}}{k},$$

% where $k<m$. Let $P_1=\{p_{11},...,p_{1j}\}(j<m)$ denote the set of positive contributing features indexed in $Z_1$ and $N_2=\{n_{21},...,n_{2l}\}(l<m)$ denote the set of negative contributing features indexed in $Z_2$. The anisotropic intersection rate can be calculated as:

% $$o=min(k,min(l,j))$$
% $$Sim_{ani}=\frac{P_1[1:o]\cap{N_2[1:o]}}{o}$$

==> sections/stable_faithfulness.tex <==
\section{Relationship between Stability and Faithfulness}\label{sec:stability}

\begin{figure}[t]
    \setlength{\abovecaptionskip}{4pt}
    \setlength{\belowcaptionskip}{0pt}
    \centering
	\includegraphics[width=0.42\textwidth]{figs/vis_manipulate_img.pdf}
	\caption{Example of manipulate attack. \re{The target explanation is that the important features are only present in the $4\times4$ square in the upper left corner.}}\label{fig:vis_manipulate_img}
	\vspace{-2mm}
\end{figure}

\re{Based on prior studies, stable explanations guarantee that if a given input is perturbed within an $\epsilon$ range and the output variance of the model is not substantial, the corresponding explanations will remain stable~\cite{robustnessxai,METFA,greedyrobustness}. Stable explanations could avoid random dominance in generating test data, yet they may not always uphold faithfulness~\cite{stablexai}. However, it's unclear how explanations should respond to larger changes in data that may lead to significant variations in model outputs. Trend tests provide in-distribution samples that can cause significant changes in model outputs and can assess faithfulness in this case.}

\re{To explore the relationship between stability and faithfulness of explanation methods, we conduct a manipulate attack on the explanation methods based on Dombrowski \etal~\cite{manipulate}. For a given target explanation $I^t$, target model $\mathcal{F}$ and original data $X$, a manipulated data $X_{ADV}$ should satisfy the following properties: (1) the model outputs of $X_{ADV}$ and $X$ should be as similar as possible, \ie $\mathcal{F}(X)\approx\mathcal{F}(X_{ADV})$ and (2) the explanation results of $X_{ADV}$ and the target explanation $I^t$ should be as similar as possible, \ie $I(\mathcal{F},X_{ADV})\approx I^t$. We achieve this manipulation attack by optimizing the following objective function: }
\re{$$\gamma_1\Vert\mathcal{F}(X)-\mathcal{F}(X_{ADV})\Vert^2+\gamma_2 \Vert I^t-I(\mathcal{F},X_{ADV})\Vert^2,$$}

\vspace{-4mm}
\noindent
\re{where $\gamma_1$ and $\gamma_2$ are tunable parameters that control the balance between the two terms. The first term aims to minimize the difference between the model outputs of $X_{ADV}$ and $X$, while the second term aims to minimize the difference between the explanation results of $X_{ADV}$ and the target explanation $I^t$.}

\begin{figure}[t]
    \setlength{\abovecaptionskip}{4pt}
    \setlength{\belowcaptionskip}{0pt}
    \centering
	\includegraphics[width=0.45\textwidth]{figs/manipulate_exp_loss.pdf}
 	\caption{MSE between explanation results and target explanations. A lower MSE means a higher similarity. Black-box explanation methods are harder to manipulate than white-box explanation methods.}\label{fig:manipulate_exp_loss}
	\vspace{-2mm}
\end{figure}

\begin{figure}[t]
    \setlength{\abovecaptionskip}{4pt}
    \setlength{\belowcaptionskip}{0pt}
    \centering
	\includegraphics[width=0.45\textwidth]{figs/manipulate_img_loss.pdf}
	\caption{MSE between perturbed images and original images. A lower MSE means a higher similarity. Manipulating IG causes greater perturbation in the image than Saliency.}\label{fig:manipulate_img_loss}
	\vspace{-2mm}
\end{figure}

\re{When attacking gradient-based explanation methods, it is necessary to compute second-order derivatives ($\nabla I(\mathcal{F},X_{ADV})$) for the model input. However, the second-order derivatives of ReLU are 0, resulting in gradient disappearance issue during optimization. To address this problem, we replace the ReLU layers in the model with softplus layers, which are given by $softplus_\beta(X)=\frac{1}{\beta}log(1+e^{\beta X})$. The softplus function is a smooth approximation to the ReLU function, with the accuracy of the approximation controlled by the $\beta$ parameter. Larger $\beta$ values yield more precise approximations to ReLU. In our experiments, we find that $\beta=30$ produces effective attack results. Since some explanation methods are not differentiable, we use the perturbation data generated by Saliency or IG to attack them, following the approach of \etal~\cite{manipulate}. In our manipulation attack, Grad and IG serve as direct attacks, while the other methods are indirect attacks. Our targets are the ResNet18 models trained on the CIFAR-10 and Tiny ImageNet datasets. Figure~\ref{fig:vis_manipulate_img} provides an example of our attack. Detailed parameter settings are available in Appendix~\ref{subsec:para_manipulation_attack}. During the manipulation attack, we measure the mean squared difference between the explanation results of the manipulated data and the target explanations, as well as the mean squared difference between the manipulated data and the original data. Our results are presented in Figure~\ref{fig:manipulate_exp_loss} and Figure~\ref{fig:manipulate_img_loss}, where a smaller mean squared difference indicates greater similarity.}

\re{Our findings reveal that manipulation attacks can affect most explanation methods, even when using indirect attacks. Black-box methods are typically more challenging to manipulate than white-box methods, possibly because the explanation results of black-box methods are more dissimilar from those of white-box methods, making the indirect attack more difficult, thus requiring more iterations to converge to the desired result. Among the methods examined, Occlusion displays higher stability and faithfulness, but it is computationally expensive and barely scalable. In the white-box methods, IG or indirect attacks using IG induce more significant variation in model output than Saliency or indirect attacks using Saliency. IG is more stable than Saliency when subjected to manipulation attacks. Based on our empirical findings, explanation methods with higher faithfulness (IG and SG-SQ-IG) are more stable when faced with manipulation attacks, but can still be successfully manipulated by increasing the perturbation budget. Therefore, developing an explanation method with both high faithfulness and high stability is a crucial research direction for the future.}

==> sections/taxonomy.tex <==
\section{Taxonomy of Local Explanations}\label{sec:taxonomy}

% \begin{figure*}
% 	\centering
% 	\includegraphics[width=0.8\textwidth]{figs/explanation_overview.pdf}
% 	\caption{An overview of explanation methods.}\label{fig:explanation_overview}
% \end{figure*}


% To gain a comprehensive understanding of the state-of-the-art explanation methods, we conducted an extensive survey of the literature. We collected papers from well-known conferences and journals, covering both the security community (\eg, IEEE S\&P, CCS, USENIX Security, NDSS, TIFS, TDSC, Euro S\&P) and the artificial intelligence (AI) community (\eg, ICML, CVPR, NIPS, ICCV, ICLR, AAAI, IJCAI, ACL, KDD, TPAMI, IJCV) in the past seven years. 
% We also used the keywords related to explanation such as ``interpretability", ``explanation", ``understanding", ``rational" to identify highly cited papers. % papers and included those with high citation rates. 
% As aforementioned, we focus on local explanations. That is, the methods provide an explanation only for a specific instance. 
% In sum, 61 papers were collected and studied. 
%We also focus on topics related to interpretability in these venues. In addition, we survey papers that cite or are cited by the aforementioned papers, and we include them if they have high citation rates.

%According to the types of algorithms that the explanation methods could be applied, 
\hjw{\sout{As mentioned above, we focus on local explanation methods in this paper.}} Local explanation methods can be either model-specific or model-agnostic. We show the taxonomy of them in Figure~\ref{fig:explanation_overview}. If one explanation method is dependent on the hyper-parameters and weights of the model,
% restricted to a specific family of machine learning algorithms, 
it is model-specific. Otherwise, it is model-agnostic. Below we introduce them in detail. 

%In general, we divide these articles into explanation methods for model inputs and for the model itself. In this paper, we will focus on explanation methods for model inputs, categorizing and measuring them. In particular, we categorize explanation methods for model inputs into model-specific and model-agnostic methods based on the accessible knowledge. 

% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.5\textwidth]{figs/interpretability}
% 	\caption{A generic process of input interpretability}\label{fig:interpretability}
% \end{figure}

%The approaches of explaining the input mainly consist of black-box methods that require only access to black-box methods that require only access to the model inputs and outputs and white-box methods that require all access to the model.

\subsection{Model-specific Explanation}\label{sec:modelspecific}

% \begin{table*}[htb]
% \scriptsize
% 	\centering
% 	\caption{Overview of MSE and BP rule. Intervention refers to whether to modify the model architecture or not.}\label{tab:mse}
% \begin{tabular}{ccccccc}
% \hline
% \textbf{MSE} & \textbf{BP Rule} & \textbf{Intervention} & \textbf{Reference Input} & \textbf{Training} & \textbf{Feature Granularity} & \textbf{Applicable Model} \\ \hline
% Saliency map~\cite{Grad} & Gradient & - & - & - & Same as input & MLP, CNN, RNN \\
% Integrated Gradient~\cite{IG} & Gradient & - & \Checkmark & - & Same as input & MLP, CNN, RNN \\
% SmoothGrad~\cite{SmoothGrad} & Gradient & - & - & - & Same as input & MLP, CNN, RNN \\
% LRP~\cite{lrp} & Layer-wise Relevance & - & \Checkmark & - & Same as input & MLP, CNN, RNN \\
% DeepLIFT~\cite{DeepLIFT} & Propagating Activation Differences & - & \Checkmark & - & Same as input & MLP, CNN, RNN \\
% Grad-CAM~\cite{GradCAM} & Gradient & - & - & - & Coarse-grained & CNN \\
% DeconvNet~\cite{Occlusion} & Transposed Convolution & - & - & - & Coarse-grained & CNN \\
% GuidedBP~\cite{GuidedBP} & Transposed Convolution & - & - & - & Coarse-grained & CNN \\
% CAM~\cite{cam} & Automatic learning & \Checkmark & - & \Checkmark & Coarse-grained & CNN \\
% Attention Mechanism~\cite{ATTN} & Automatic learning & \Checkmark & - & \Checkmark & Same as input & MLP, CNN, RNN \\
% Natural Language~\cite{generatevizexplanation,improvinginterpretabilityofdnnwithsemanticinfo} & Automatic learning & \Checkmark & - & \Checkmark & Coarse-grained & MLP, CNN, RNN \\ \hline
% \vspace{-4mm}
% \end{tabular}
% \end{table*}

Model-Specific Explanation (MSE) methods treat a model as a white box and have full access to the model's internal structure (\eg, weights of each layer). To explain a given input instance, MSE methods recognize important features through the internal operations of the model. Backpropagation (BP) rules are often used to mark features that highly impact the output. Below is the formal definition of MSE.

%The Model-Specific Explanation(MSE) takes a model as white box with full access to the model information. MSE attempts to leverage the information at each layer of the model, analyzing the correlation between outputs and inputs from the last to the input layer of the model. In short, the core of MSE is to find the correlation between outputs and inputs by backpropagation (BP) rules. One way is to formulate BP rules artificially; another way is to exploit learning ability of the machine learning model by adding explanation modules that learn the BP rules automatically during training. We have distilled the core ideas of MSE and defined it as follows:

% \todo{Provide a formal definition for this line of approaches.}
\begin{mydef}\label{def:mse}
	\textbf{(Model-specific Explanation)} Given a model $\mathcal{F}(\mathbf{X})$ and an input instance $\mathbf{X}$, MSE is to find the importance score $\phi$ for the features in $\mathbf{X}$. Formally, $\phi = I(\mathbf{X}, \mathcal{F})$,
	where $I$ is the BP rules that calculate the correlation between the output $\mathcal{F}(\mathbf{X})$ and the input $\mathbf{X}$. $I$ is dependent on the $\mathcal{F}$ and $\mathbf{X}$.
	%A MSE is defined as follows: 
	%$$I_i(o_{i+1}, f_i, w_i, b_i, o_i)=\phi_i,$$ 
	%where $o_i$ and $\phi_i$ have the same dimension. $I$ is the core algorithm of MSE whose basic idea is to calculate the correlation between output and input layer by layer from output to input. $I$ can utilize the complete information of the model, including inputs, outputs, model architecture and model parameters. $\phi_i$ is the contribution values of each neuron in i-th layer. $\phi_0$ is the importance score of each features in $X$.
\end{mydef}

% A typical algorithm $I$ to calculate importance score $\phi$ uses BP rules. Suppose $\phi^{(i)}$ represents the importance score of the layer $i$. Then $\phi^{(i)}$ can be calculated using the nonlinear function $f^{(i)}$ as follows: $\phi^{(i)} = I^{(i)}(o^{(i-1)}; f^{(i)}, w^{(i)}, b^{(i)})$. $I^{(i)}$ is the MSE method operating the layer $i$. $o^{(i-1)}$ is the input of layer $i$ while the output of layer $i$ is $o^{(i)}=f^{(i)}(w^{(i)}o^{(i-1)}+b^{(i)})$, where $w^{(i)}$ and $b^{(i)}$ are the weights and the bias of the layer $i$, respectively. $o^{(0)}$ is the input of layer $1$, \ie $o^{(0)}=\mathbf{X}$. $o^{(0)}_j$ represents the j-th feature of $o^{(0)}$. Starting from the last layer $n$, the algorithm $I=(I^{(1)}, I^{(2)}, ..., I^{(n)})$ can back-propagate the output and finally get $\phi$.
	
%The output of the layer $i$ is denoted as $o_i=f_{i-1}(w_{i}o_{i-1}+b_i)$, where $w_i$ and $b_i$ are the weights and the bias of the layer $i$, respectively. 

% \begin{table*}[htb]
% 	\scriptsize
% 	\centering
% 	\caption{Overview of MAE methods. The first column shows the MAE methods. The second and third column present different ways to mutate input and measure output drift. The last column shows whether the MAE method has adversarial example mitigation. E is exhaustive mutation, R denotes random mutation and O denotes optimization mutation. P is class probability. $\Delta{P}$ denotes the change in class probalitiy and LM indicates using the linear model as the surrogate model.}\label{tab:mae}
% 	\begin{tabular}{ccccccc}
%     \hline
%     \textbf{MAE} & \textbf{IM} & \textbf{Identification} & \textbf{Train} & \textbf{Feature Granularity} & \textbf{Mask Params} & \textbf{AE Mitigation} \\ \hline
%     Occlusion~\cite{Occlusion} & E & P & - & Same as stride & \Checkmark & - \\
%     Fong \etal ~\cite{MeaningfulPerturbation} & O & $\Delta{P}$ & - & Same as input & - & \Checkmark \\
%     Dabkowski \etal ~\cite{RealtimeSaliency} & O & $\Delta{P}$ & \Checkmark & Same as input & - & \Checkmark \\
%     LIME~\cite{LIME} & R & LM & \Checkmark & User defined & \Checkmark & - \\
%     LEMNA~\cite{LEMNA} & R & LM & \Checkmark & User defined & \Checkmark & - \\
%     SHAP~\cite{SHAP,lshapley,i-Algebra} & E, R & $\Delta{P}$ & - & User defined & \Checkmark & - \\ \hline
%     \vspace{-4mm}
% 	\end{tabular}
% \end{table*}


According to the way that $I$ calculates the $\phi$, MSE can be further divided into two types: \textit{non-interventional MSE (n-MSE)} and \textit{interventional MSE (i-MSE)}. n-MSE does not change the model and calculates $\phi$ by defining a set of rules for different layers. I-MSE needs to change the model (\eg, add additional layers) and train/tune the model so that the newly added layers automatically learn the rules. %We introduce the details below. 
% We compare these methods through several properties and summarize the comparison in Table~\ref{tab:mse}.


%We classify MSE into two categories: Artificially Designated Explanation Rule (ADER) and Automatic Learning Explanation Rule (ALER). An overview of MSE is shown in Table~\ref{tab:mse}.

\vspace{2mm}
\noindent\textbf{Non-interventional MSE (n-MSE).} 
The n-MSE methods do not require changes or retraining of the model. Instead, by defining a set of BP rules for different layers in the model, the n-MSE methods can calculate $\phi$ backward from the last layer. Saliency map is a typical n-MSE method that defines the $I$ using the gradients.
% , \hjw{\ie, $I^{(i)}_j = \delta{o^{(i)}}/\delta{o^{(i-1)}_j}, I_j=\prod_{i=1}^{n}I^{(i)}_j=\delta{o^{(n)}}/\delta{o^{(0)}_j}$.} 
% Its underlying assumption is that the gradient of the feature reflects the feature’s influence on model output. 
% In other words, a feature with a larger gradient has a greater impact on the output. 
Although simple and easy to implement, Saliency map suffers from the gradient saturation problem and is sensitive to noise. Integrated gradient (IG)~\cite{IG} moderates the gradient saturation problem by 
% introducing a baseline input $\mathbf{x’}$. Then IG 
considering the straight-line path from the baseline input $\mathbf{x’}$ to the input $\mathbf{x}$ and computes the gradients at all points along the path. 
% To calculate $\phi$, IG calculates integrated gradient by cumulating the computed gradients along the path.
% \hjw{$$I_j=(x_j-x'_j)\int_{\alpha=0}^{1}\frac{\delta{o'^{(n)}}}{\delta{o^{(0)}_j}}d\alpha,$$
% where $o'^{(0)}=x'+\alpha\times(x-x')$.} 
SmoothGrad~\cite{SmoothGrad} tries to reduce the sensitivity of the gradient by adding Gaussian noise to the input
% \hjw{($o^{(0)}=X+\mathcal{N}(0,\sigma^2)$, where $\mathcal{N}(0,\sigma^2)$ represents Gaussian noise with standard deviation $\sigma$)} 
and then calculating the average of the gradients. Grad-CAM~\cite{GradCAM} and its variants~\cite{gradcam++,scorecam,fullgrad} leverage the gradients and feature maps of the last convolutional layer to
% . The feature maps of the last convolutional layer are weighted and summed, and then upsampled to the same shape as the input to obtain a heat map with the importance scores of features. In this way, Grad-CAM
produce a coarse heat map highlighting the important regions in the image.
Deep Learning Important FeaTures (DeepLIFT)~\cite{DeepLIFT} alleviates the gradient saturation by using the difference between the input and the reference point to explain the importance of input features.
% But, the choice of it is important and affects the explanation performance.
% Even when the gradient is zero, the difference with the reference point allows information to be propagated. In this way, 
% The vanishing gradient problem could be alleviated by the reference point, but
% . Depending on the choice of different BP rules, DeepLIFT may be able to better capture the dependencies between features~\cite{SHAP}. According to the design of DeepLIFT, 
% the choice of it is important and affects the explanation performance.
% In addition to the aforementioned gradient-based BP rule, Deconvolutional Network (DeconvNet)~\cite{Occlusion} and GuidedBP~\cite{GuidedBP} use transposed convolution as the backpropagation rule. In order to understand the convolution operation, it is necessary to explain the feature activation of the intermediate convolutional layers. Therefore, DeconvNet and GuidedBP use the transposed convolution operation to map the activations back to the input space. DeconvNet only retains features with positive gradients and discards features with negative gradients, while GuidedBP only retains features with positive gradients and activations. GuidedBP generates sharper visualization of descriptive image regions.
% Bach \etal ~\cite{lrp} believes that there is no direct correlation between the gradient and the model output.
% , and that calculating the gradient requires a reference input other than the target input.
Bach \etal ~\cite{LRP} produce Layer-wise Relevance Propagation (LRP), which does not require the calculation of gradient or reference input by decomposing the output of the layer backward and preserving the correlation. 
% Therefore, applying LRP rules layer-by-layer from the output to the input can obtain the correlation between the output and the input, \ie, the contribution of input features to the output. 
% Compared with gradient-based methods, 
% LRP does not require differentiable or smooth neuron activation. 
Marco \etal~\cite{sensitivityn} prove that LRP is equivalent to input-weighted Saliency map and DeepLIFT when certain conditions are satisfied. 

% Shrikumar \etal ~\cite{lrpeq} argues that the model output on target label $F_{target}(\mathbf{X_i})$ at test point $\mathbf{X_i}$ is not directly related to the derivative $\frac{\delta{F_{target}(\mathbf{X_i})}}{\delta{\mathbf{X_i}}}$. They produce Layer-wise Relevance Propagation (LRP) which proposes rules to decompose importance score of neuron output into each input of neuron based on the inputs' value. LRP is equivalent to an element-wise product between the saliency map and the input without modification for numerical stabilization. LRP focus on the explanation of the target point $\mathbf{X_i}$ with respect to the reference point $F_{target}(\mathbf{X_0})=0$ . However, the gradient calculated by Saliency map may point to the local optimum with the same sign as $F_{target}(\mathbf{X_i})$, which does not satisfy the objective of LRP.

\vspace{2mm}
\noindent\textbf{Interventional  MSE  (i-MSE).} 
I-MSE aims to allow the model to learn the rules for mapping the output to the important features in the input. The typical method is to modify the model architecture (e.g., add a new layer as the explanation module) and retrain/tune the model. In this process, the added module can learn mapping rules. Zhou \etal ~\cite{cam} propose CAM to explain CNN by adding a global average pooling layer (GAP) to learn the weight of each feature map of the last convolutional layer.
% The input of GAP is the feature maps output by the last convolutional layer. GAP outputs the average value of each feature map, weighs these values, and sends them to the last layer (i.e., fully connected layer) for classification. The weights can be learned during training. Then, 
Then, for an input instance, CAM upsamples the feature maps 
% output by the last convolutional layer
to the same size as the model input, and uses the learned weights to form the explanation results. Unfortunately, not all models are compatible with GAP, which makes the design of Grad-CAM~\cite{GradCAM} become popular.
%ALER requires modifying model architecture and training, the basic idea is to add explanation module to the model. The earliest emergence of ALER is CAM for explaining CNN proposed by Zhou et al~\cite{cam}. CAM adds a global average pooling layer (GAP) to the last convolutional layer, whose input is all feature maps of the last convolutional layer and output is the average of each feature map. The output of the GAP is input to the last fully connected layer (FC) used for classification. The weight of the FC is used as the weight of each feature map. These feature maps are weighted and summed, which is a linear fusion operation.  And then they are upsampled to the same size as the model input, and this is the final explanation result. Unfortunately, not all models are adapted to GAP. Thus Grad-CAM~\cite{GradCAM}, which does not require modification of the model architecture, is proposed and replace CAM.
Another modification on models is to add the attention module~\cite{ATTN}. It aims to learn feature contribution by assigning different weights to each feature of the input
% . The attention value serves as feature contribution
~\cite{seq2seq,transformer}. 
% However, Sofia \etal ~\cite{isattninterpretable} find that the attention mechanism often fails to recognize the most important features for model prediction. Jain \etal ~\cite{attnisnotexplanation} identify that randomly assigned attention weights have a similar effect on model prediction, which demonstrates that the attention values contribute little to the explanation. But Sarah \etal ~\cite{attnisnotnotexplanation} further reveal that the samples obtained from the adversarial search used in ~\cite{attnisnotexplanation} are out of distribution. 
% However, attention-based methods may not be able to identify the important features of the input~\cite{isattninterpretable, attnisnotexplanation, attnisnotnotexplanation}. 
% Recent studies provide natural language (NL) explanations for model decisions. Usually, they use labeled images with NL explanations for training, combined with additional language module to learn natural language explanations~\cite{generatevizexplanation,improvinginterpretabilityofdnnwithsemanticinfo,vqae}. 

% In short, backpropagation rules are the core of MSE. MSE needs to design different backpropagation rules according to different neural network layers. As they make full use of the model information, including architecture, parameters, etc., MSE methods are generally more efficient and have higher faithfulness than MAE methods that require sampling and approximation.

% We also evaluate this in Section~\ref{}.

%Although the CAM which need to modify model architecture has been replaced, attention mechanism~\cite{ATTN} has received increasing attention in recent years. Attention mechanism can help to extract more critical information by giving different weights to each part of the input, so that the model can make more accurate judgments. Attention mechanism can be used as the explanation of feature importance. The basic idea of the attention-based ALER is to exploit the attention mechanism in the model to explain itself automatically, taking the attention values as the feature contributions. However, it is controversial whether the attention mechanism correctly reflects the feature contributions. Jain \etal ~\cite{attnisnotexplanation} finds that randomly assigned attention weights only have a small effect on the model's prediction. Sofia \etal ~\cite{isattninterpretable} finds that the attention mechanism often cannot identify those features that are most important for model prediction by masking features with high attention weights. Sarah \etal ~\cite{attnisnotnotexplanation} refutes Jain \etal ~\cite{attnisnotexplanation} by arguing that the samples obtained from the adversarial search used in Jain \etal ~\cite{attnisnotexplanation} are out of distribution, so that the generated samples have no practical meaning and therefore could not prove the effectiveness of the adversarial search. In conclusion, although attention-based methods have low computational cost, they have significant limitation that the attention weights do not guarantee the validity of explanation results.

% Recent studies provide natural language (NL) explanations for model decisions. Usually, they use labeled images with NL explanations for training, combined with additional language models to learn natural language explanations. 
% Hendricks \etal ~\cite{generatevizexplanation} use the Caltech UCSD Birds 200-2011 (CUB), an image classification dataset with NL explanations to generate descriptions of important features that influence the model’s decision. They use an LRCN framework~\cite{LRCNframework}, which consists of a CNN~\cite{cnn} used to extract features and two stacked LSTMs~\cite{lstm} used to generate descriptions. 
% Similarly, Dong \etal~\cite{improvinginterpretabilityofdnnwithsemanticinfo} use the encoder-decoder framework. The encoder consists of a CNN and a bi-directional LSTM~\cite{bilstm} to extract video features with semantic information. It then passes the output of the encoder into an LSTM decoder to generate natural language explanations. Dong \etal~\cite{improvinginterpretabilityofdnnwithsemanticinfo} and VQA-E~\cite{vqae} extend NL explanation to image captioning and question-and-answer tasks. 
% A recent study~\cite{multimodelexplanation} combines attention mechanism with NL explanations, called multi-model explanation. 
% NL explanation is easy for humans to understand, but requires datasets with natural language descriptions for training.


%In addition to providing attention-based explanations, some studies can also give natural language (NL) explanations for model decisions. Typically, they usually use labeled images with NL explanations for training and incorporate additional language models to learn natural language explanations. 
%Hendricks et al.~\cite{generatevizexplanation} use the Caltech UCSD Birds 200-2011 (CUB) which is an image classification dataset with NL explanation to learn NL explanation automatically by using an LRCN framework~\cite{LRCNframework} which consists of a CNN~\cite{cnn} for extracting features and two stacked LSTMs~\cite{lstm} for generating descriptions of important features that influence model's decision. Similarly, \cite{improvinginterpretabilityofdnnwithsemanticinfo} uses an encoder-decoder framework, where the encoder consists of a CNN and a bi-directional LSTM~\cite{bilstm} for extracting video features with semantic infomation, and then pass the encoder's output into the LSTM decoder to generate natural language explanation. \cite{improvinginterpretabilityofdnnwithsemanticinfo} and VQA-E~\cite{vqae} extend NL explanation to image captioning and question-and-answer task. NL explanation requires datasets with category-distinctive natural language descriptions, which is unrealistic for most cases. 

%Multi-model explanation~\cite{multimodelexplanation} requires the inclusion of an attention mechanism for scoring feature importance and LSTM module for generating natural language explanation in the model architecture. Multi-model explanation can simultaneously generate feature importance scores based on the attention mechanism and NL explanation based on the language model. Obviously, Multi-model explanation will also face the problems of attention-based and language-based methods.

%MSEs establish output-to-input correlations by ADERs or ALERs. MSEs dependent on specific model architecture and require training. Each ADER has its own rationale and concerns, but none of them can be theoretically proven to be directly related to the model behavior. ALERs attempt to exploit uninterpretable model to explain another uninterpretable model, which seems to be stuck in a infinite loop and is controversial so far.

% They can be grouped into two classes: %, which are divided into two types according to whether the model needs to be modified or not: 
% the first one is reversed-based methods that calculate the importance scores of features using customized back-propagation rules without modifying model architecture; the second one is self-explanation methods that modify a model by adding an interpretation module, usually an attention layer or a language model so that the model learns to be an interpreter automatically during training.

%\subsection{Black-box Methods}
\subsection{Model-agnostic Explanation}\label{sec:modelagnostic}

Model-agnostic Explanation (MAE) could be applied to any machine learning algorithm. It attempts to establish a connection between input instances and corresponding outputs by treating the model as a black box and ignoring its internal model architectures and weights. 
% A typical explanation way is to mutate the features of an instance and observe the changes of the output.
% From input-output pairs, explanation methods could identify the most important features that affect the model’s decision.
%These input-output pairs can be further mapped through explanation methods. 
Below we formally define MAE.

%Model-agnostic Explanation (MAE) takes a machine learning model as a black box without accessing its internals such as architecture and weights. 
%%The black-box methods have restricted access to model information and can only find mapping relationships from the input and output. 
%The basic idea is to perturb the features of an input to generate a set of perturbed inputs which is then used to analyze the effect of perturbations on the output of the model.

% \todo{Provide a formal definition for this line of approaches.}
\begin{mydef}\label{def:mae}
	\textbf{(Model-agnostic Explanation)} Given an input instance $\mathbf{X}\in{\mathbb{R}^{p\times{q}}}$, a model $\mathcal{F}$, a mask matrix $\mathbf{M}\in(0,1)^{p\times{q}}$, $\mathcal{F}_{target}(\mathbf{X})\in[0,1]$ represents the probability that the model $\mathcal{F}$ classifies $\mathbf{X}$ as the target label. The goal of an MAE is as follows:
	$$\arg\max_{\mathbf{M}}(\mathcal{F}_{target}(\mathbf{X})-\mathcal{F}_{target}(\mathbf{M}\odot \mathbf{X}))\cdot{\sum_{\substack{1\leq{i}\leq{p}\\1\leq{j}\leq{q}}}\mathbf{M_{ij}}}$$
\end{mydef}

% \todo{There are three essential components in this type of approaches. How to mutate input, what result got from the model, and how to explain the changes. }

The first part maximizes the distance between the model output after masking the features and the original data model output. The second part ensures that the retained features are as much as possible. The features that are masked are the important features. The operation $\mathbf{M}\odot \mathbf{X}$ is the input mutation that multiplies $\mathbf{X}$ with $\mathbf{M}$ element-wise. $\mathcal{F}_{target}$ measures the output drift. Although the basic ideas of MAE methods are similar, they are different in terms of input mutation, output drift and the way to weigh features. 
% We compare these methods through these aspects and summarize the comparison in Table~\ref{tab:mae}.

%We distill three key steps from the existing MAE: input mutation, output drift and explanation. The overview of MAE is shown in Table~\ref{tab:mae}

\vspace{2mm}\noindent\textbf{Input Mutation and Output Drift}. 
Since the optimization problem in Definition~\ref{def:mae} is difficult to solve, researchers have proposed several methods to mutate the input (i.e., find the mask $\mathbf{M}$). The straightforward solution is to generate all possible masks (a.k.a. \textit{exhaustive mutation}). For example, 
% Occlusion~\cite{Occlusion} proposes to mask the input image with a moving square to generate perturbed samples. The square slides from the first pixel of the image to the last pixel. Both the stride of sliding and the size of the square are specified by the user. 
% In this way, the $\sum_{\substack{1\leq{i}\leq{p}\\1\leq{j}\leq{q}}}M_{ij}$ is fixed. So the user only needs to choose the mask that minimizes $F_{target}(M\odot X)$, which can be directed calculated by feeding the perturbed samples into the model and comparing the outputs. 
SHAP leverages the exhaustive mutation to calculate Shapley values~\cite{SHAP}. Although exhaustive mutation is precise, the computational cost is prohibitive. 
% If there are $F$ binary features, the number of different combination of features is $2^{F}$. 
%The input mutation includes two forms: exhaustive mutation and random mutation. Exhaustive mutation requires the exhaustive enumeration of all possible combinations. Occlusion~\cite{Occlusion} proposes to mask the original input image with a moving square to generate perturbed samples. This square will slide from the first pixel to the last pixel of the image in a user-specified stride. The precise calculation of the Shapley value in SHAP method also requires an exhaustive enumeration of all feature combination cases~\cite{SHAP}. Suppose there are $F$ binary features and for each feature contribution, we must to calculate $2^{(F-1)}$ feature combination cases.
To improve the efficiency, prior research proposes \textit{random mutation}, which only provides a subset of the perturbed samples ($\mathbf{M}\odot \mathbf{X}$) from exhaustive mutation. 
% Because of its high efficiency, researchers often adopt this method in the explanation. 
Shapley value can be estimated using random mutation~\cite{ShapleySampling,shapleyregression,quantitativeinputinfluence}. Occlusion~\cite{Occlusion} chooses to use moving squares whose size is specified by the user.
% Different methods vary from the features to mutate. 
%Regarding the features to mutate, different methods may vary. 
% The basic idea is to treat each pixel as feature~\cite{MeaningfulPerturbation, RealtimeSaliency}. However, the generated results is hard to understand by humans, and the computational cost is very high.
LIME~\cite{LIME} and LEMNA~\cite{LEMNA} leverage random mutation and superpixel segmentation~\cite{slicsuperpixels} to improve efficiency. Although superpixel segmentation has more semantic information for humans, it may not conform to the model, making the explanation results lose faithfulness (see Section~\ref{sec:measurement}). 
% Although random mutation works more efficiently, the distribution of the perturbed inputs may differ from the distribution produced by exhaustive mutation, making the explanation results inaccurate. To further solve this problem, researchers guide the input mutation process by optimizing the objective function in Definition~\ref{def:mae}, which is called \textit{optimization mutation}. Fong \etal ~\cite{MeaningfulPerturbation} and Dabkowskiet \etal ~\cite{RealtimeSaliency} propose the idea of iterative optimization to generate the perturbations. 
% The difference is that it needs to optimize the objective function for each input to generate mutation samples in \cite{MeaningfulPerturbation}, while \cite{RealtimeSaliency} trains a model to automatically generate mutation samples. 
% It shows that \cite{RealtimeSaliency} is more efficient than~\cite{MeaningfulPerturbation} for generating a larger number of mutation samples.

%It is obvious that the exhaustive mutation has high computational cost. Therefore, random mutation, which also can specify condition, is more often adopted. We can use random mutation to estimate the Shapley value, which is more practical~\cite{ShapleySampling,shapleyregression,quantitativeinputinfluence}. LIME~\cite{LIME} and LEMNA~\cite{LEMNA} adopt random mutation as well. 

% Different methods vary from the features to mutate. 
% %Regarding the features to mutate, different methods may vary. 
% The basic idea is to treat each pixel as feature~\cite{MeaningfulPerturbation, RealtimeSaliency}. However, the generated results is hard to understand by humans, and the computational cost is very high. Occlusion~\cite{Occlusion} chooses to use moving squares and lets the user specify the size of the square. LIME~\cite{LIME} uses superpixel segmentation~\cite{slicsuperpixels}, which is a cluster of pixel values based on color similarity and proximity in the image plane. Although superpixel segmentation has more semantic information for humans, it may not conform to the model, making the explanation results lose faithfulness (see Section~\ref{subsec:traditionnalparams}). 
%We train a ResNet18~\cite{resnet} on the CIFAR-10 dataset~\cite{cifar10} and then used LIME to explain the test data fed into it. We choose the number of superpixel segments from 10 to 50 with stride of 10. We find that the average intersection of LIME's explanation across different superpixel segments is 35.84\%, which implies that some explanation may be unfaithful to the model behavior.\kai{add more studies here and compare them.}


%The granularity of the features they use can be different from the original input. For image data, superpixel segmentation can be used in advance to cluster pixels values based on their color similarity and proximity in the image plane~\cite{slicsuperpixels}. Superpixel segmentation is equivalent to dimension reduction and therefore simplifies the combination of mutations. The risk is that superpixel segmentation results conform to human cognition but may not conform to model cognition, reducing the faithfulness of the explanation to the model.

%Further, it is more efficient and specific to guide the input mutation by optimizing the objective function, which is called optimization mutation. Fong \etal ~\cite{MeaningfulPerturbation} and Dabkowskiet \etal ~\cite{RealtimeSaliency} propose to generate semantic perturbation by iterative optimization. The difference is that Fong \etal ~\cite{MeaningfulPerturbation} needs to optimize the objective function for each input in order to generate mutation sample. Dabkowskiet \etal ~\cite{RealtimeSaliency}, on the other hand, trains a model that automatically generates mutation samples, which is more efficient than  ~\cite{MeaningfulPerturbation} when generating a larger number of mutation samples. 

The output drift describes the impact of input mutation, reflecting the model’s behavior. There are two main methods for measuring the output drift: class probability and class label. Occlusion~\cite{Occlusion} and SHAP-based methods~\cite{SHAP,lshapley,i-Algebra} record the difference of the class probability for each perturbed sample to measure the output drift. 
% Fong \etal ~\cite{MeaningfulPerturbation} and Dabkowskiet \etal ~\cite{RealtimeSaliency} incorporate the class probability into the objective function. 
LIME~\cite{LIME} and LEMNA~\cite{LEMNA} record whether the class label of the perturbed sample changes. 
% For example, if the output label of the perturbed sample changes, $F_{target}(M\odot X)=0$; otherwise, $ F_{target}(M\odot X)=1$.

\vspace{2mm}\noindent\textbf{Identifying important features.} 
After constructing input-output pairs, the explanation methods will weigh the features and identify the most important features.
% , which should be easy for humans to understand and conform to the model. 
Occlusion~\cite{Occlusion} directly uses the target classification probability as the metric. The lower the probability caused by the mutated input, the more important the features. 
% This method is easy to implement, but the result is susceptible to the parameters such as stride and mask size. 
% In addition, the features obscured by a square mask may not be objects that humans can understand.
%The explanation step attempts to model the importance of the input features using information on input mutation and output drift. Modeling feature importance can be viewed as a quantitative process. The simplest approach is to directly treat the target classification probability as a quantitative metric, as is the case for Occlusion~\cite{Occlusion}. The more the target classification probability decreases, the higher the importance of the features mutated. Occlusion is not only computationally expensive but also very sensitive to the stride and the size of the mask. The input covered by the square mask is not unnatural and irrational to human. 
% LIME~\cite{LIME} and LEMNA~\cite{LEMNA} leverage self-explanatory models to establish the connection between input mutation and output drift. 
Based on the local linearity assumption of the neural network decision boundary, LIME~\cite{LIME} and LEMNA~\cite{LEMNA} train a surrogate linear model using the perturbed data and labels to establish the connection between input mutation and output drift. The weights of the linear model reflect the importance of the feature. LEMNA uses a mixture regression model and the fused lasso constraint to improve the explanation accuracy.
SHAP~\cite{SHAP}, derived from cooperative game theory, calculates Shapley values as feature importance and recommends combining the assumptions of the current additive feature attribution methods (such as LIME) to approximate calculation. 
% So far, a series of different explanation frameworks have been constructed with SHAP values~\cite{lshapley,i-Algebra}.

%Further, we can automate the modeling, one way is to model the data pairs of input mutation to output drift with a self-explanatory model, as done in LIME~\cite{LIME} and LEMNA~\cite{LEMNA}. Based on the assumption of local linearity at the decision boundary of the neural network, LIME and LEMNA train a surrogate linear model with the perturbed data and labels. The weights of the linear model represent the importance scores. LEMNA extends the LIME method to security applications from two aspects: enhancing the explanation accuracy by using mixture linear model and considering the continuous dependence of features by using fused lasso constraint.

%In particular, SHAP~\cite{SHAP}, derived from cooperative game theory, calculate Shapley values as feature importance using data pairs of input mutation and output drift. This is a special automatic modeling approach that draws on cooperative game theory. To effectively identify the influential features, SHAP suggests incorporating the assumptions of feature independence and model local linearity to approximate the calculation using current additive feature attribution methods such as LIME, LEMNA, etc. So far, there have been a series of different interpretation frameworks built with SHAP values~\cite{lshapley,i-Algebra}.

% Another way to identify important features is to use a generative model. Fong \etal~\cite{MeaningfulPerturbation} propose to generate semantic perturbation by iterative optimization with the objective function in Definition~\ref{def:mae}, where the position and shape of the mask are correlated with the target category. 
% However, optimization takes a long time and may introduce overfitting masks. It also takes a long time to avoid generating adversarial samples. Dabkowski \etal~\cite{RealtimeSaliency} train a U-Net model~\cite{unet} based on the optimization goal in Definition~\ref{def:mae} for saliency map prediction. It only needs one forward calculation to obtain the saliency map, which is more than an order of magnitude faster and more accurate than ~\cite{MeaningfulPerturbation}. In order to avoid generating overfitting masks,
% % the introduction of extra features by unsmoothed masks, 
% Dabkowski \etal~\cite{RealtimeSaliency} improve the smoothness of the mask through the average and total variation penalty.

% In sum, MAE explains an input instance without accessing the internals of the model. Exhaustive mutation considers the combinations of all features and is faithful to the model, but at the same time, it is impractical due to the high cost. To solve this problem, most MAE methods use random mutation, numerical optimization, and dimension reduction to improve efficiency and simplify feature combinations. However, incomplete sampling and the introduction of human' prior knowledge may lead to a decrease in faithfulness, which is also experimentally verified in Section~\ref{sec:measurement}.

% A more detailed development of MAE is presented below. Occlusion~\cite{Occlusion} proposes to mask the original input image with a moving square to generate perturbed samples, using heat maps to represent the variation in confidence with different masking locations. 
% The value of each position on the heat map is the confidence score on the original input category for the perturbed sample with a square masking on that position. Occlusion is not only computationally expensive but also very sensitive to the stride and size of the mask. 
% However, the feature covered by the square mask is not natural and rationale to human. 
% To address this problem, Fong \etal~\cite{MeaningfulPerturbation} propose to generate semantic perturbation by iterative optimization, where the position and shape of the mask are correlated with the target class. 
% However, the optimization takes over long time and may introduce overfitting masks, requiring a large cost to avoid generating adversarial samples. Dabkowski \etal~\cite{RealtimeSaliency} train a model for saliency map prediction. It requires only a single forward calculation to obtain a saliency map, which is more than an order of magnitude faster and more accurate than ~\cite{MeaningfulPerturbation}. In order to avoid the introduction of extra features by unsmoothed masks, \cite{RealtimeSaliency} improves the smoothness of the mask via a total variation penalty.

% Based on the assumption of local linearity at the decision boundary of the neural network, a dataset consisting of perturbed samples can also be used to fit an interpretable surrogate model which acts as an approximation to the target model. Local Interpretable Model-agnostic Explanations (LIME) method is to train a surrogate linear model by generating perturbation samples over a small domain and querying the target model to obtain the labels of perturbation samples~\cite{LIME}. LEMNA~\cite{LEMNA} extends the LIME method to security applications from two aspects: enhancing the interpretation accuracy and considering the continuous dependence of features. For the former, LEMNA uses mixture linear models to improve the accuracy of surrogate model fitting, and for the latter, LEMNA applies fused lasso constraints when fitting the surrogate models to capture the continuous dependence of features.

% SHAP~\cite{SHAP} proposes a framework to unify LIME, DeepLIFT~\cite{DeepLIFT}, LRP~\cite{LRP}, and Classic Shapley Value Estimation~\cite{ShapleySampling,shapleyregression,quantitativeinputinfluence}. Derived from the cooperative game theory, SHAP can theoretically guarantee that additive feature attribution methods have unique solution. SHAP uses the Shapley value of the original model's conditional expectation as the feature importance score. Assuming that the data have $F$ binary features, it is difficult to calculate the SHAP values directly by considering all $2^F$ cases.
% To effectively identify the influential features, SHAP suggests incorporating the assumptions of feature independence and model local linearity to approximate the calculation using current additive feature attribution methods such as LIME, LEMNA, etc. So far, there have been a series of different interpretation frameworks built with SHAP values~\cite{lshapley,i-Algebra}.

% \textit{In summary, MAE usually have to generate a number of perturbed samples, making them computationally inefficient and ignore feature dependencies. Additionally, the quality of perturbed samples affect the explanation significantly.}

%\subsection{White-box Methods}

